A Multigrid Method for CutFEM and its Convergence

We develop a convergence theory for geometric multigrid with vertex-patch smoothers applied to cut finite element discretizations of the Poisson problem. The framework addresses non-inherited level forms and the mismatch between the physical and active domains. Using the discrete extension property, we prove two-level convergence bounds uniform in the mesh size and the cut geometry, and W-cycle bounds under an additional smallness assumption on the two-level rate. The numerical experiments intentionally use the stronger V-cycle, for which no convergence bound is claimed here. The convergence constants degrade with the degree $p$. Lowering the ghost penalty improves iteration counts. An aligned two-cell model exhibits a semidefiniteness threshold of order $p^{-2}$, whereas the visibility scale of a degree-$p$ cut mode decreases exponentially. Experiments at the model threshold reduce the iteration counts, but do not establish an assembled-operator threshold.

==> scripts.tex <==
% Command to execute data extraction script
\newcommand{\executeextract}[3]{%
    \ifrunscripts
        % #1: input csv file
        % #2: SQL query
        % #3: output data file
        \immediate\write18{python3 scripts/extract_data.py --input "#1" --query "#2" --output "#3"}%
    \fi
}

% Example: configure extracts/plots by copying or updating these lines
% \executeextract{results/...}{SELECT ...}{results/tmp/...}


==> splitted/preamble.tex <==
% Load a package only if the class 'acmart' is NOT loaded.
% Usage: \LoadPackageUnlessAcm[<options>]{<package>}
\makeatletter
\newcommand{\LoadPackageUnlessAcm}[2][]{%
    \@ifclassloaded{acmart}{%
        % acmart is loaded -> skip the package (informational message)
        \PackageInfo{preamble}{Skipping package `#2' because acmart class is used}%
    }{%
        % acmart not loaded -> load package (with or without options)
        \if\relax\detokenize{#1}\relax
            \usepackage{#2}%
        \else
            \usepackage[#1]{#2}%
        \fi
    }%
}
\makeatother

\LoadPackageUnlessAcm{caption}
\LoadPackageUnlessAcm{subcaption}
\LoadPackageUnlessAcm{authblk}
\LoadPackageUnlessAcm{hyperref}

% elsarticle-style captions: small, bold "Figure/Table N." label, period separator.
\makeatletter
\@ifclassloaded{acmart}{}{
    \captionsetup{
        font=small,
        labelfont=bf,
        labelsep=period,
        justification=justified,
        singlelinecheck=false,
        skip=8pt
    }
}
\makeatother

% elsarticle-style tables: small font for table content.
\usepackage{etoolbox}
\AtBeginEnvironment{tabular}{\small}

% amsthm before any \newtheorem; shared.tex loads it again later, harmlessly
\usepackage{amsthm}
\newtheorem{hypothesis}{Hypothesis}

\usepackage{amstext}
\usepackage{stmaryrd}
\usepackage{algpseudocode}

\usepackage{units}
\usepackage{cancel}
\usepackage{graphicx}

\usepackage{xcolor}
\usepackage{array}
\usepackage{verbatim}
\usepackage{booktabs}
\usepackage{makecell}
\usepackage{calc}
\usepackage{textcomp}
\usepackage{multirow}
\usepackage{tikz,tikzscale}

\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{pgfkeys}
\pgfplotsset{compat=1.18}

\definecolor{deepgreen}{RGB}{0,100,0}

\newif\ifrunscripts
\runscriptstrue
\input{scripts.tex}

\pgfplotsset{
    p2/.style={teal, mark=*},
    p3/.style={orange, mark=triangle*},
    p4/.style={red, mark=pentagon*},
    p5/.style={violet, mark=otimes*},
    p7/.style={blue, mark=square*},
}

\newcommand{\plotwidth}{0.49\columnwidth}
\newcommand{\plotheight}{0.4\columnwidth}

\pgfplotscreateplotcyclelist{paper markers}{
    {teal,    solid, mark=*},
    {orange,   solid, mark=triangle*},
    {blue,     solid, mark=square*},
    {red,      solid, mark=pentagon*},
    {violet,     solid, mark=otimes*},
    {brown,    solid, mark=halfcircle*},
    {black,   solid, mark=diamond*},
}

\newcommand{\PaperColorA}{teal}
\newcommand{\PaperColorB}{orange}
\newcommand{\PaperColorC}{blue}

\colorlet{BarColorOne}{orange!60!white}
\colorlet{BarColorTwo}{teal!80!white}
\colorlet{BarColorThree}{red!80!black}
\colorlet{BarColorFour}{blue!60!white}
\colorlet{BarColorFive}{brown!70!black}

\pgfplotsset{legend swatch/.style={area legend, draw=none}}
\newcommand{\RangeFillOpacity}{0.15}

\pgfplotsset{
    paperplot/.style={
            width=\plotwidth,
            height=\plotheight,
            cycle list name=paper markers,
            every axis/.append style={font=\small},
            grid=major,
            thick
        }
}

\pgfplotsset{
    longplot/.style={
            width=0.8\columnwidth,
            height=\plotheight,
            cycle list name=paper markers,
            every axis/.append style={font=\small},
            grid=major,
            thick
        }
}

\usepackage[all]{xy}
\usepackage{mathtools}
\usepackage{enumitem}
\usepackage{placeins}
\usetikzlibrary{calc}
\usetikzlibrary{shadings}
\usepgfplotslibrary{fillbetween}

\usepackage[mode=multiuser,status=draft]{fixme}
\fxsetup{innerlayout=inline}
\fxsetup{targetlayout=colorcb}
\fxusetheme{color}
\FXRegisterAuthor{mw}{envmw}{MW}

\definecolor{apply}{rgb}{0.3,.7,0.}
\definecolor{applyface}{rgb}{.9,.95,0.}
\definecolor{invert}{rgb} {0.5,0.,1.}
\colorlet{invertface}{invert!60!red}

% Toggle print-friendly TODO notes; use \printversionfalse for screen colors.
\newif\ifprintversion
\printversiontrue

\usepackage[colorinlistoftodos,prependcaption,textsize=small]{todonotes}
\ifprintversion
    \setuptodonotes{
        backgroundcolor=white,
        linecolor=black,
        bordercolor=black,
        textcolor=black
    }
\fi

\newcommand{\FigureSubst}[1]{ \fbox{
        \begin{minipage} {0.7\textwidth} #1
        \end{minipage}    }   }

\def\mesh{\mathbb M}
\def\cell{K}
\def\R{\mathbb R}
\def\Q{\mathbb Q}
\def\ncol{N_{\text{colors}}}
\def\resth#1{I_{#1}^{\downarrow_{h}}}
\def\prolh#1{I_{#1}^{\uparrow_{h}}}

\def\prol#1{I^\uparrow_{#1}}
\def\rest#1{I^\downarrow_{#1}}

\def\prolp#1{I_{#1}^{\Uparrow_{p}}}
\def\restp#1{I_{#1}^{\Downarrow_{p}}}

\def\vertices{\mathbb V}
\def\vertex{X}
\def\vA{\mathbf{A}}
\def\vQ{\mathbf{Q}}
\def\vb{\mathbf{b}}
\def\vx{\mathbf{x}}
\def\vy{\mathbf{y}}

\usepackage{colortbl}
\newcommand{\myrowcolor}{\rowcolor[gray]{0.925}}
\newcommand{\headercolor}{\rowcolor[gray]{0.825}}
\usepackage{booktabs}
\usepackage[font=footnotesize,position=b]{subcaption}
\usepackage{adjustbox}

\newcommand{\pluseq}{\stackrel{+}{\gets}}

\newcommand{\LUpNew}{local_update}
\newcommand{\LSolNew}{local_solve}

\newcommand{\residual}{r}
\newcommand{\res}{\text{res}}

\makeatletter
\def\pgfplots@getautoplotspec into#1{%
        \begingroup
        \let#1=\pgfutil@empty
        \pgfkeysgetvalue{/pgfplots/cycle multi list/@dim}\pgfplots@cycle@dim
        %
        \let\pgfplots@listindex=\pgfplots@numplots
        %%% Start new code
        \pgfkeysgetvalue{/pgfplots/cycle list set}\pgfplots@listindex@set
        \ifx\pgfplots@listindex@set\pgfutil@empty
        \else
            \c@pgf@counta=\pgfplots@listindex
            \c@pgf@countb=\pgfplots@listindex@set
            \advance\c@pgf@countb by -\c@pgf@counta
            \globaldefs=1\relax
            \edef\setshift{%
                \noexpand\pgfkeys{
                    /pgfplots/cycle list shift=\the\c@pgf@countb,
                    /pgfplots/cycle list set=
                }
            }%
            \setshift%
            \globaldefs=0\relax
        \fi
        %%% End new code    
        \pgfkeysgetvalue{/pgfplots/cycle list shift}\pgfplots@listindex@shift
        \ifx\pgfplots@listindex@shift\pgfutil@empty
        \else
            \c@pgf@counta=\pgfplots@listindex\relax
            \advance\c@pgf@counta by\pgfplots@listindex@shift\relax
            \ifnum\c@pgf@counta<0
                \c@pgf@counta=-\c@pgf@counta
            \fi
            \edef\pgfplots@listindex{\the\c@pgf@counta}%
        \fi
        \ifnum\pgfplots@cycle@dim>0
            \c@pgf@counta=\pgfplots@cycle@dim\relax
            \c@pgf@countb=\pgfplots@listindex\relax
            \advance\c@pgf@counta by-1
            \pgfplotsloop{%
                \ifnum\c@pgf@counta<0
                    \pgfplotsloopcontinuefalse
                \else
                    \pgfplotsloopcontinuetrue
                \fi
            }{%
                \pgfkeysgetvalue{/pgfplots/cycle multi list/@N\the\c@pgf@counta}\pgfplots@cycle@N
                \pgfplotsmathmodint{\c@pgf@countb}{\pgfplots@cycle@N}%
                \divide\c@pgf@countb by \pgfplots@cycle@N\relax
                %
                \expandafter\pgfplots@getautoplotspec@
                \csname pgfp@cyclist@/pgfplots/cycle multi list/@list\the\c@pgf@counta @\endcsname
                {\pgfplots@cycle@N}%
                {\pgfmathresult}%
                \t@pgfplots@toka=\expandafter{#1,}%
                \t@pgfplots@tokb=\expandafter{\pgfplotsretval}%
                \edef#1{\the\t@pgfplots@toka\the\t@pgfplots@tokb}%
                \advance\c@pgf@counta by-1
            }%
        \else
            \pgfplotslistsize\autoplotspeclist\to\c@pgf@countd

            \pgfplots@getautoplotspec@{\autoplotspeclist}{\c@pgf@countd}{\pgfplots@listindex}%
            \let#1=\pgfplotsretval
        \fi
        \pgfmath@smuggleone#1%
        \endgroup
    }

\pgfplotsset{
    cycle list set/.initial=
}
\makeatother

% Typeset all floating tables (body and caption) in footnote size.
\AtBeginEnvironment{table}{\footnotesize}
\AtBeginEnvironment{table*}{\footnotesize}

